Learning Synergistic Attention for Light Field Salient Object Detection

We propose a novel Synergistic Attention Network (SA-Net) to address the light field salient object detection by establishing a synergistic effect between multi-modal features with advanced attention mechanisms. Our SA-Net exploits the rich information of focal stacks via 3D convolutional neural networks, decodes the high-level features of multi-modal light field data with two cascaded synergistic attention modules, and predicts the saliency map using an effective feature fusion module in a progressive manner. Extensive experiments on three widely-used benchmark datasets show that our SA-Net outperforms 28 state-of-the-art models, sufficiently demonstrating its effectiveness and superiority. Our code is available at https://github.com/PanoAsh/SA-Net.

==> figures/table_data.tex <==
\multirow{8}{*}{{4D}}	
    &	Ours	&	\textbf{0.920}	&	\textbf{0.918}	&	\textbf{0.954}	&	\textbf{0.032}	&	\textbf{0.736}	&	\textbf{0.784}	&	\textbf{0.849}	&	\textbf{0.078}	&	\textbf{0.844}	&	\textbf{0.841}	&	\textbf{0.889}	&	\textbf{0.074}	\\
~	&	ERNetT~\cite{Piao2020ExploitARERNet}	&	{0.889}	&	{0.899}	&	{0.943}	&	{0.040}	&	0.705	&	0.777	&	{0.831}	&	0.082	&	{0.842}	&	{0.838}	&	\textbf{0.889}	&	{0.080}	\\%Results_From_Original_Paper
~	&	ERNetS~\cite{Piao2020ExploitARERNet}	&	0.838	&	0.848	&	0.916	&	0.061	&	0.651	&	0.736	&	0.824	&	0.085	&	0.721	&	0.726	&	0.820	&	0.137	\\%Results_From_Original_Paper
~	&	{DLFS}~\cite{DUTMV}	&	0.801	&	0.841	&	0.891	&	0.076	&	0.615	&	0.741	&	0.783	&	0.098	&	0.715	&	0.737	&	0.806	&	0.147	\\%Results_From_ERNet_Paper
~	&	LFS$^{\star}$~\cite{li2017saliency}	&	0.484	&	0.563	&	0.728	&	0.240	&	0.430	&	0.579	&	0.686	&	0.205	&	0.740	&	0.680	&	0.771	&	0.208	\\%Results_From_ERNet_Paper
~	&	MCA$^{\star}$~\cite{HFUT}	&	-	&	-	&	-	&	-	&	-	&	-	&	-	&	-	&	0.815	&	0.749	&	0.841	&	0.150	\\%Results_From_ERNet_Paper
~	&	WSC$^{\star}$~\cite{Li2015WSC}	&	-	&	-	&	-	&	-	&	-	&	-	&	-	&	-	&	0.706	&	0.706	&	0.794	&	0.156	\\%Results_From_ERNet_Paper
~	&	DILF$^{\star}$~\cite{Zhang2015SaliencyDILF}	&	0.641	&	0.705	&	0.805	&	0.168	&	0.555	&	0.695	&	0.736	&	0.131	&	0.728	&	0.755	&	0.810	&	0.168	\\%Results_From_ERNet_Paper
\hline	

\multirow{7}{*}{{3D}} 
    & S2MA~\cite{LiuS2MA} & 0.754 & 0.787 & 0.841 & 0.103 & 0.647 & 0.761 & 0.787 & 0.100 & 0.819 & 0.837 & 0.863 & 0.095  \\
~   & D3Net~\cite{fan2020rethinking} & 0.790 & 0.822 & 0.869 & 0.084 & 0.692 & 0.778 & 0.827 & 0.080 & 0.804 & 0.825 & 0.853 & 0.095 \\
~   &	CPFP~\cite{zhao2019contrast}	&	0.730	&	0.741	&	0.808	&	0.101	&	0.594	&	0.701	&	0.768	&	0.096	&	0.524	&	0.599	&	0.669	&	0.186	\\
~	&	TANet~\cite{Chen2019TANet}	&	0.771	&	0.803	&	0.861	&	0.096	&	0.638	&	0.744	&	0.789	&	0.096	&	0.804	&	0.803	&	0.849	&	0.112	\\
~	&	MMCI~\cite{Chen2019MMCI}	&	0.750	&	0.785	&	0.853	&	0.116	&	0.645	&	0.741	&	0.787	&	0.104	&	0.796	&	0.799	&	0.848	&	0.128	\\
~	&	PDNet~\cite{zhu2019pdnet}	&	0.763	&	0.803	&	0.864	&	0.111	&	0.629	&	0.770	&	0.786	&	0.105	&	0.780	&	0.786	&	0.849	&	0.116	\\
~	&	PCA~\cite{chen2018progressively}	&	0.762	&	0.800	&	0.857	&	0.100	&	0.644	&	0.748	&	0.782	&	0.095	&	0.801	&	0.807	&	0.846	&	0.112	\\
%~	&	CTMF~\cite{Han2017CTMF}	&	0.790	&	0.823	&	0.881	&	0.100	&	0.620	&	0.752	&	0.784	&	0.103	&	0.791	&	0.801	&	0.856	&	0.119	\\
%~	&	DF~\cite{qu2017rgbd}	&	0.733	&	0.716	&	0.838	&	0.151	&	0.562	&	0.670	&	0.742	&	0.138	&	0.756	&	0.751	&	0.816	&	0.162	\\
\hline	

\multirow{4}{*}{{2D}} 
     & F3Net \cite{wei2020f3net} & 0.882 & 0.888 & 0.900 & 0.057 & 0.718 & 0.777 & 0.815 & 0.095 & 0.797 & 0.806 & 0.824 & 0.106 \\
~   & GCPANet~\cite{GCPANet} & 0.867 & 0.885 & 0.898 &  0.064 & 0.691 & 0.777 & 0.799 & 0.105 & 0.805 & 0.822 & 0.809 & 0.097\\ 
~   &	EGNet~\cite{zhao2019egnet}	&	0.870	&	0.886	&	0.914	&	0.053	&	0.672	&	0.772	&	0.794	&	0.094	&	0.762	&	0.784	&	0.776	&	0.118	\\
%~	&	CPD~\cite{feng2019attentive}	&	0.887	&	0.890	&	0.923	&	0.050	&	0.689	&	0.764	&	0.810	&	0.097	&	0.841	&	\textbf{0.846}	&	0.865	&	0.083	\\
~	&	PoolNet~\cite{liu2019simple}	&	0.868	&	0.889	&	0.919	&	0.051	&	0.683	&	0.776	&	0.802	&	0.092	&	0.769	&	0.800	&	0.786	&	0.118	\\
%~	&	PAGRN~\cite{zhang2018progressive}	&	0.828	&	0.822	&	0.878	&	0.084	&	0.635	&	0.717	&	0.773	&	0.114	&	0.725	&	0.727	&	0.805	&	0.147	\\
%~	&	C2S~\cite{li2018contour}	&	0.791	&	0.844	&	0.874	&	0.084	&	0.650	&	0.763	&	0.786	&	0.111	&	0.749	&	0.806	&	0.820	&	0.113	\\
%~	&	R$^{3}$Net~\cite{deng2018r3net}	&	0.783	&	0.819	&	0.833	&	0.113	&	0.625	&	0.727	&	0.728	&	0.151	&	0.781	&	0.789	&	0.838	&	0.128	\\
%~	&	Amulet~\cite{zhang2017amulet}	&	0.805	&	0.847	&	0.882	&	0.083	&	0.636	&	0.767	&	0.760	&	0.110	&	0.757	&	0.773	&	0.821	&	0.135	\\
%~	&	UCF~\cite{zhang2017learning}	&	0.769	&	0.837	&	0.850	&	0.107	&	0.623	&	0.754	&	0.764	&	0.130	&	0.710	&	0.762	&	0.776	&	0.169	\\
%~	&	SRM~\cite{wang2017stagewise}	&	0.832	&	0.848	&	0.899	&	0.072	&	0.672	&	0.762	&	0.801	&	0.096	&	0.827	&	0.826	&	0.863	&	0.099	\\
%~	&	NLDF~\cite{luo2017non}	&	0.778	&	0.786	&	0.862	&	0.103	&	0.636	&	0.729	&	0.807	&	0.091	&	0.748	&	0.745	&	0.810	&	0.138	\\
%~	&	DSS~\cite{hou2017deeply}	&	0.728	&	0.764	&	0.827	&	0.128	&	0.626	&	0.715	&	0.778	&	0.133	&	0.644	&	0.677	&	0.749	&	0.190	\\

